Monte Carlo Variational Auto-Encoders

Variational auto-encoders (VAE) are popular deep latent variable models which are trained by maximizing an Evidence Lower Bound (ELBO). To obtain tighter ELBO and hence better variational approximations, it has been proposed to use importance sampling to get a lower variance estimate of the evidence. However, importance sampling is known to perform poorly in high dimensions. While it has been suggested many times in the literature to use more sophisticated algorithms such as Annealed Importance Sampling (AIS) and its Sequential Importance Sampling (SIS) extensions, the potential benefits brought by these advanced techniques have never been realized for VAE: the AIS estimate cannot be easily differentiated, while SIS requires the specification of carefully chosen backward Markov kernels. In this paper, we address both issues and demonstrate the performance of the resulting Monte Carlo VAEs on a variety of applications.

==> ais_iwae.tex <==
\subsection{Multi-sample AIS VAE}

We now take interest in a multi sample AIS IWAE, writing 
\begin{equation}
\elbo =  \int \sum_{\chunk{a}{1}{K}}  \prod_{j=1}^n q_\phi(z_0^{(j)}\mid x) \prod_{t=1}^K \alpha^{a_t}_{t,u_t} \bigl( \Circ{i=1}{t-1} \propmap{i, u_i}^{a_i} (z_0^{(j)})\bigr)  \densinnovation(u_t) \log\left(\frac{1}{n}\sum_{j=1}^n \prod_{t=0}^{K}  w_t(\Circ{i=1}{t} \propmap{i, u_i}^{a_i} (z_0^{(j)}))\right)\rmd z_0^{(1:n)} \rmd \chunk{u}{1}{K}\eqsp.
\end{equation}

Write, for simplicity, $\bw(z, \chunk{a}{1}{K}, \chunk{u}{1}{K}) = \prod_{t=0}^{K}  w_t(\Circ{i=1}{t} \propmap{i, u_i}^{a_i} (z))$, and similarly $\bar{\alpha}(z, \chunk{a}{1}{K}, \chunk{u}{1}{K}) = \prod_{t=1}^K \alpha^{a_t}_{t,u_t} \bigl( \Circ{i=1}{t-1} \propmap{i, u_i}^{a_i} (z)\bigr)$.

The, we can write (by an ugly notation which won't please the readers here but I lack ideas)
\begin{equation}
\elbo = \PE_{z, u, a}\left[\log\left(\frac{1}{n}\sum_{j=1}^n \bw(z^{(j)}, \chunk{a}{1}{K}^{(j)}, \chunk{u}{1}{K}^{(j)})\right)\right]\eqsp.
\end{equation}

==> ais_vae.tex <==
% !TEX root = main.tex

\subsection{Annealed Importance Sampling VAE}
  We recall here the notions of \Cref{subsec:ais_estimator} for defining the Annealed Importance Sampling VAE, AIS VAE.
   Let $\{M_{t, x}\}_{t = 1}^K$
  %,\{L_{t,x}\}_{t=0}^{K-1}$ 
  be a family of Markov kernels associated to the proposal mappings $\{\propmap{t, u, x}\}_{1 \leq t \leq K, u \in \msu}$, the acceptance functions $\{\alpha_{t,u,x}\}_{1 \leq t \leq K, u \in \msu}$, and the innovation noise with density $\densinnovation$, such that for each $1 \leq t\leq K$, $M_{t, x}$ is $\unnormdistr_{t, x}$-reversible.
  The main difference \wrt\ the previous section is that we consider here Accept/Reject (A/R) steps, modelled by the acceptance functions, to ensure the reversibility of our approach.
  Thus, we now rely on the AIS identity~\eqref{eq:weights_ais}.
  By simplicity of notation, we now omit the dependency in $x$ of these quantities. Note that these quantities also depend on some parameters, also denoted $\phi$ in the following, which can be optimized
  \arno{might be worth adding something like e.g. the temperature schedule or the variance of the proposals to illustrate what we mean}. Define the bound for AIS
  %We can define the weight functions $w_{t}= \unnormdistr_{t+1,x}/\unnormdistr_{t,x}$, such that for any $(x,z)\in\rset^{d\times P}$, 
  %$\log w_{t}(z) = (\beta_{t+1}-\beta_t)(\log p_\theta(x,z)-\log q_\phi(z\mid x))$, and finally, define the objective of the AIS VAE
  \begin{multline}
    \elboais(\theta, \phi; x) = \int \sum_{\chunk{a}{1}{K}} q_\phi(z_0 \mid x) \prod_{t = 1}^K \alpha^{a_t}_{t, u_t} \bigl(\Circ{i = 1}{t - 1} \propmap{i, u_i}^{a_i} (z_0)\bigr) \\
    \densinnovation(u_t)
    \log\left(\prod_{t = 1}^{K} w_t\bigl(\Circ{i=1}{t-1} \propmap{i, u_i}^{a_i} (z_0)\bigr)\right)\rmd z_0 \rmd \chunk{u}{1}{K}\eqsp.
  \end{multline}
  %
  This objective is now straightforward to estimate and optimize. 
  The expression of the gradients is given in supplementary. Note that we can easily estimate this quantity by sampling  $z_0 \sim q_\phi(\cdot \mid x)$, $\chunk{u}{1}{K} \sim h$, and recursively for $1\leq t\leq K$, $a_t \sim \Ber\bigl(\alpha_{t, u_t}(z_{t - 1})\bigr)$, $z_t = \propmap{t, u_t}^{a_t}(z_{t - 1})$. 


==> differentiable_markov.tex <==
% !TEX root = main.tex

==> experiments.tex <==
Consider now observations $x\in\rset^P$, typically high dimensional ($P\gg 1$). We specify a latent variable model, that is, we assume the existence of some latent variables $z\in\rset^D$, with $D<P$ typically, and the likelihood model, parameterized by $\theta$,
\begin{equation}
p_\theta(x) = \int p_\theta(x\mid z) p_\theta(z)\rmd z\eqsp,
\end{equation}
where the conditional generative model $p_\theta(x\mid z)$ is parameterized by a deep neural network, and $p_\theta(z)$ is some prior on the latent space, with typically  $p_\theta(z)=p(z)$. 


In turn, we present the results of the SMC versions of the VAE presented above.
In the following, let $K$ be the number of annealing steps performed in the SIS estimator, 
and write the annealing schedule as $0=\beta_0<\dots<\beta_{K+1}= 1$, and for $0\leq t\leq K+1$, $\unnormdistr_{t,x}(z)=\unnormdistr_t(z\mid x) = q_\phi(z\mid x)^{1-\beta_t} p_\theta(x,z)^{\beta_t}$.


\subsection{Toy example}
  In order to prove efficiency of our approach compared to competitors, we consider a toy hierarchical example for variational inference.
  Assume some data $x\in\rset^p$, with $p=1$ here, is generated from the latent variables $z \in \rset^d$, with $d=2$ with the following scheme. Let $\eta$ be in $\rset^+_*$. Sample $z\sim \Normal(0; \Id)$, $x = \eta * \|z\| + \epsilon$, where $\epsilon\sim\Normal(0, \sigma^2)$. 
  This defines the likelihood of $x$ given $z$, and we can thus perform Variational Inference. We parameterize an initial density $q$ as a function of some parameters $\phi$ and $x$ (this example is directly inspired from amortized variational inference performed in VAE), and perform various schemes of VI: we compare the schemes described above, both using AIS identity (MALA kernels) and using kernel densities (ULA kernels), to classical Variational Inference with mean-field approximation, to Variational Inference with IWAE bound, and to Variational inference with flows (using Real-valued Non-Volume Preserving transformation - RealNVP, \cite{dinh2016density}). 
  \begin{figure}
    \centering
    \renewcommand{\arraystretch}{0.1}
    \begin{tabular}{ccc}
      \hspace{-10pt}\includegraphics[width=0.33\linewidth]{pics/circle_true_posterior.png} & \hspace{-20pt}\includegraphics[width=0.33\linewidth]{pics/circle_vae_posterior.png} & \hspace{-20pt}\includegraphics[width=0.33\linewidth]{pics/circle_iwae_posterior.png} \\
      \hspace{-10pt}\includegraphics[width=0.33\linewidth]{pics/circle_flows_rnvp5_posterior.png} & \hspace{-20pt}\includegraphics[width=0.33\linewidth]{pics/circle_ais_posterior.png} & \hspace{-20pt}\includegraphics[width=0.33\linewidth]{pics/circle_ula_posterior_2.png}
    \end{tabular}
    \caption{Visualization of the posterior approximation given after optimization of different bounds for toy generation process. Top row, from left to right: True posterior, VAE posterior, IWAE posterior. Bottom row, from left to right: VI with RealNVP posterior, VI with AIS posterior, VI with SIS/ULA posterior}
     \label{fig:toy_example_posterior}
  \end{figure}

  This aims at showing the superiority in flexibility and in form of the SMC enhanced Variational inference, which proves more efficient than IWAE algorithms, and more flexible directly than flows enhanced VI. 
  \achille{input some graph with figures directly here ? when learning eta parameter, for example ? or like HVAE ?}
  
  We also demonstrate this impression quantitatively by reproducing the experiment of \cite{caterini:doucet:2018}.
  
 



\subsection{Parameters of the model}

Crucial parameters to tune in our models are the stepsizes of the different transitions, both for the AIS and the Langevin VAE, as well as the annealing schedule.

The stepsize $\stepsize$ is chosen for AIS such that the A/R procedure accepts in average to a proportion chosen around $\rho $. The quantity $\rho$ is an hyperparameter of our problem and in our experiments, we usually choose $\rho = 0.7$.
Moreover, it has proven effective to choose a different stepsize over the dimensions. To this end, we write $\mathbf{\stepsize}$ to be a vector of size $\rset^p$, and adapt it with the following heuristic
\begin{equation}
    \mathbf{\stepsize} = 0.9 \mathbf{\stepsize} + 0.1 \stepsize /(\epsilon+ \operatorname{std}\nabla p_\theta(x,z))\eqsp,
\end{equation}
where $\operatorname{std}$ denotes the standard deviation over the batch $x$ of the quantity $\operatorname{std}\nabla p_\theta(x,z)$, and $\epsilon >0$. This quantity, computed for the Langevin transitions, rules the geometry of the latent space we are considering. This allows us to take smaller moves on the regions where the potential can be very steep. It is inspired in particular by the Adam heuristics \cite{kingma2014adam}.
We use a similar heuristic for SIS, computing as well what would the output of an A/R procedure would be. We tune stepsize on a similar fashion, except now targetting a value $\rho=0.9$ (this ensures that we stay ``almost reversible''), thus allowing us to keep a low variance SIS estimator).


The choice of the temperature schedule $\{\beta_k\}_{k=0}^K$ is complex, and we have focused on three different situations in the following. First, consider the temperature schedule fixed and regularly spaced between 0 and 1. Second,consider the parameter $\alpha_0\in(0,1)$, learnable, and write the quadratic tempering scheme, for $k\leq K$, $\beta_k = ((1- \alpha_0) k^2/K^2 + \alpha_0)^{-2}$, following \cite{caterini:doucet:2018}.
Finally, we consider a scheme where all $\{\beta_k\}_{k=0}^K$ are directly learnable. 




\subsection{Numerical results}

Following \cite{wu:burda:grosse:2016}, we propose to evaluate our models using AIS.

We choose as a base distribution the distribution output by the encoder, and perform $K$ steps of annealing to compute the estimator of the likelihood, as given by \eqref{eq:SiS-estimator-Z}.
In practice, we use $K=10$ HMC steps for evaluating our models, with $N=1000$ samples. 
The numerical results are presented in table...


==> introduction.tex <==
% !TEX root = main.tex

%%% First talk about generative models
***This is just a draft, to lay out plan of the intro***


The development of Variational Inference (VI) has been crucial for  scalable unsupervised learning, generative models, and in high dimensional sampling. It differs from classical Markov chain Monte Carlo (MCMC), which aims at creating a chain of $N$ samples, which will be arbitrarily close to a target distribution as $N \rightarrow \infty$ under mild conditions. However, MCMC suffers from some limitations, for example, the chain must reach an equilibrium to be close to the target distribution, which is typically hard to assess, especially in high dimensions. 
VI, on the other hand, scales well with dimension, as one can draw easily samples from the variational distribution. However, it introduces a bias of approximation of the target by the variational distribution.
In amortized VI, \citep{kingma:welling:2014}, such an approximation error can lead to poorer performance results.
Indeed, VAE are classically learnt using an proxy estimate of the marginal log-likelihood $p_\theta(x) = \int p_\theta(x,z)\rmd z$ where $x\in\rset^N$ is some data, typically high dimensional, and $z\in\rset^d$ is some latent variable. Introducing an auxiliary variational distribution $q_\phi(z\mid x)$, the set of parameters $\{\theta, \phi\}$ is  learnt during optimization of the Evidence Lower Bound (ELBO) defined as\textcolor{red}{Arno: remove $x$ from the ELBO? unncessary}
\begin{multline}
\label{eq:elbo}
  \elbo(\theta, \phi)= %\PE_{q_\phi}\left[\log\left(\frac{p_\theta(x,z)}{q_\phi(z\mid x)}\right)\right] = 
  \int \log\left(\frac{p_\theta(x, z)}{q_\phi(z \mid x)}\right) q_\phi(z \mid x) \rmd z\eqsp\\
   =\log p_\theta(x) - \KL\bigl(q_\phi(z \mid x) ~\|~ p_\theta(z \mid x)\bigr) \leq \log p_\theta(x) \eqsp.
\end{multline}
%
A lot of work has been devoted to enrich the variational distribution, in order to improve directly the quality of the approximation~\cite{rezende2015variational, kingma2016improving}.
More generally, an ELBO can be constructed using any positive unbiased estimator $\hat{p}_\theta(x)$ of the loglikelihood $p_\theta(x)$ as noticed by \cite{mnih2016variational} as it follows from Jensen's inequality that 
\begin{align}
    \elbo(\theta, \phi) &= \mathbb{E}[\log \hat{p}_\theta(x)]\leq \log p_\theta(x)\eqsp.
\end{align}
A simple Taylor expansion shows that 
\begin{align}
    \elbo(\theta, \phi) \approx \log p_\theta(x) -\frac{1}{2}\textup{var}\left[\frac{\hat{p}_\theta(x)}{p_\theta(x)}\right] \eqsp;
\end{align}
see e.g. \cite{maddison2017filtering,domke2018importance} for formal results. Hence the ELBO becomes tighter as the variance of the estimator decreases. 

Then, another method to estimate a closer quantity to the marginal log-likelihood has been introduced in~\cite{burda:grosse:2015}. The Importance Weighted Auto Encoder (IWAE) generalizes the ELBO, and defines a proxy on the marginal log-likelihood $p_\theta(x)$ as a $K$-sample importance sampling estimate 
\begin{equation}
\label{eq:iwae_bound}
  \elbo_{\IWAE}( \theta, \phi) = \PE_{q_\phi}\left[\log\left(\frac{1}{K}\sum_{i = 1}^K \frac{p_\theta(x, z_i)}{q_\phi(z_i \mid x)}\right)\right]\eqsp.
\end{equation}
 This line of work suggests that a related issue to the optimization of VAE is thus the evaluation of decoder based generative models, in which a tractable and efficient estimator to the marginal log-likelihood is computed.


%%% Most efficient way : annealed importance sampling...
Some effort to consider efficient evaluation methods has been made by~\cite{wu:burda:grosse:2016}, using in particular Annealed Importance Sampling (AIS). AIS~\cite{neal2001annealed}, and in general Sequential Importance Sampling are Sequential Monte Carlo inspired method that provide an efficient low variant estimator of a normalizing constant.
%%%Why people can't do it
However promising AIS and SIS might be for evaluating normalizing constants~\cite{wu:burda:grosse:2016}
%A natural objective, at that point, would be to learn directly a Variational Auto Encoder with a very efficient way to compute a normalizing constant, that is Annealed Importance Sampling (in particular,  compare AIS and IWAE bounds on log-likelihood, proving effectively the relevance of an AIS based VAE).
it has proven difficult to perform VI schemes with those algorithms.
AIS includes reversible MCMC steps, which usually comes with Metropolis-Hastings correction step, notoriously difficult to differentiate. Previous attempts~\cite{salimans:kingma:welling:2015, wolf:karl:2016} usually bypass it. 
On the other hand, authors of~\cite{huang:tan:lacoste:courville:2018} consider as well annealed variational objectives and SIS schemes that they can differentiate. 
However, those methods build a looser lower bound to the likelihood as the extend on some path space, in order to get ``better'' samples from the variational approximation; see \Cref{subsec:sis_est}. This comes at an increase in computational cost and the introduction of heavily parameterized inference functions in order to guarantee a low variance estimate in the end.
%%% Introduce our claims
Our contributions to prior work in variational inference and Sequential Monte Carlo methods can be summarized as follows:
\begin{itemize}[topsep=0pt,itemsep=0pt,partopsep=1pt,parsep=1pt,listparindent=2pt,leftmargin=12pt]
%begin{itemize}
  \item \textbf{Claim 1:} We show how to develop an efficient SIS estimate of the evidence in a VI context, in particular using unadjusted Langevin dynamics.
  \item \textbf{Claim 2:} We extend this SIS estimator to the well-known Annealed Importance Sampling estimator, again in a VI context. For this theoretical contribution, we use a particular representation of Markov kernels which allows us to differentiate through them, even if they have no density (applied in particular to Metropolis-Hastings kernels).
  \item \textbf{Claim 3:} We apply these new methods to build a novel Monte Carlo VAE, and show its efficiency over real-world datasets.
\end{itemize}


==> markov_ais_vi.tex <==
% !TEX root = main.tex

\subsection{Reversible kernels and how to differentiate them}
\paragraph{Basics of Markov kernels}
A Markov kernel is $M$ is a function defined on $\rset^{d_z} \times \borel( \rset^{d_z})$ such that for any $z \in \rset^{d_z}$, $M(z, \cdot)$ is a probability distribution on $\borel(\rset^{d_z})$, \ie\ the probability starting from $z$ to hit the set $A$.
%A variety of Markov kernels can be defined. 
The simplest is ``deterministic'', in which case  $M(z,A)= \updelta_{\propmap{}(z)}(A)$, where $\propmap{}$ is a measurable mapping on $\rset^{d_z}$ and $\updelta_y$ is the Dirac mass at $y$. Instead of a single mapping $\propmap{}$, we can consider a family of ``indexed'' mappings $\set{\propmap{u}}{u \in \msu}$ where $\msu$ is the index. If $\msu \subset \rset^{d_u}$, and $\densinnovation$ is a p.d.f on $\rset^{d_U}$, we may consider $M(z,A)= \int \delta_{\propmap{u}(z)}(A) \densinnovation(u) \rmd u$. 
%Sampling from this Markov kernel is easy: 
To sample from $M$, we first sample $u \sim \densinnovation$ and then apply the mapping $\propmap{u}(z)$. If $d_z=d_u$, and if the function $G_z$ defined, for all $(z, u)$ by $G_z(u)= \propmap{u}(z)$ is a diffeomorphism, then 
\begin{multline}
\label{eq:markov-kernel-transition}
  M(z, A) = \int \indi{A}\bigl(G_z(u)\bigr) \densinnovation(u) \rmd u = 
  \int \indi{A}(z') m(z, z') \rmd z' ,\\
  \text{with} \, m(z, z')= \Jac_{G_z^{-1}}(z') \densinnovation\bigl(G_z^{-1}(z')\bigr) \eqsp,
\end{multline}
where $\Jac$ denoting the Jacobian. In this case, the Markov kernel has a transition density $m(z, z')$. This is what we describe in the previous section.
%It is worthwhile to note that all Markov kernels with a transition density  are of the form \eqref{eq:markov-kernel-transition}. 

Finally, some Markov kernels have both a  deterministic and a continuous component. This is for example the case of Metropolis-Hastings kernels, which may be expressed
\begin{equation}
\label{eq:MH-kernel}
  M(z,A) = \int \alpha(z,z') m(z,z') \indi{A}(z') \rmd z' + \bigl(1 - \bar{\alpha}(z)\bigr) \delta_z(A),
\end{equation}
where $m$ is a transition density, $\alpha(z, z') \in \ccint{0,1}$ is the acceptance function and   $\bar{\alpha}(z) = \int \alpha(z, z') m(z, z') \rmd z'$. 
Assuming that the transition density $m(z,z')$ satisfies \eqref{eq:markov-kernel-transition}, conditionally to the current state $z \in \rset^{d_z}$, we first draw $u \sim \densinnovation$, then compute $z' = \propmap{u}(z)$  
  , and for all $u\in\msu$, $\propmap{u}\colon \rset^D \to \rset^D$ is referred to as the \textit{proposal mapping}. %In this work, $\phi$ collectively denotes the parameters used in the proposal distribution, and $(U_k)$ is referred to as the \emph{innovation noise}.
 %Let $\mu_{\msu}$ be a $\sigma$-finite measure on $(\msu, \mcu)$ and $h$ the density function \wrt\ $\mu_{\msu}$ of the innovation noise.
 \\
% \emph{In order to satisfy some reversibility property}, $Y_{k + 1}$ is accepted with probability $\alpha^{\MH}\bigl(Z_k, \propmap{U_{k+1}}(Z_k)\bigr)$. 
In the Metropolis-Hastings algorithm, $\alpha\colon \rset^{2D} \to \ccint{0, 1}$ is set so that $M$ is $\pi$-reversible $
    \pi(\rmd z) M(z, \rmd z')= \pi(\rmd z')M(z', \rmd z)$.
  %
  It is crucial for the derivation below to write $M$ as
  \begin{multline}
  \label{eq:def_M}
    M(z, \msa) = \int_{\msu} \densinnovation(u) Q_u(z, \msa) \rmd u \eqsp,  \text{ where } \\
    Q_u\bigl(z, \msa\bigr) = \alpha_u(z) \updelta_{\propmap{u}(z)}(\msa) + \bigl\{1 - \alpha_u(z)\bigr\} \updelta_z(\msa) \eqsp,
  \end{multline}
  %
   with $\alpha_u(z) = \alpha\bigl(z, \propmap{u}(z)\bigr)$.
%However, in the case above where we do not necessarily want to satisfy a reversibility property, we set for any $u\in\msu$, $\alpha_u\equiv 1$.
%We write in general, in the following, these functions $\alpha_u$, which can be set to $1$ at any point if we do not consider reversible kernels.
To illustrate this definition, consider first the symmetric Random Walk Metropolis Algorithm (RWM). In such case, $\msu =\rset^D$,  and $\varphi=\densgauss$ is the $D$-dimensional standard normal density. The proposal mapping is
  \begin{equation}
    T^{\RWM}_{\phi}(z, u) = z + \Sigma_\phi^{1/2} u,
  \end{equation}
  where $\{\Sigma_\phi, \phi \in \rset^q\}$ is a parametric family of positive definite matrices, and the acceptance function is given by $\alpha^{\RWM}_{\phi}(z, u) = 1 \wedge \bigl(\pi(T^{\RWM}_{\phi}(z,u))/\pi(z)\bigr)$.

  Consider now the Metropolis Adjusted Langevin Algorithm (MALA); see~\cite{besag:1994}. Assume that $z \mapsto \log \pi(z)$ is differentiable and denote by $\nabla \log \pi(z)$ its gradient. The proposal mapping and the associated acceptance function for MALA algorithm are given by
  \begin{align}
  \label{eq:forward-transform-MALA}
    &T^{\MALA}_{\phi} (z,u) = z + \Sigma_\phi \nabla \log \pi(z)+ \sqrt{2} \Sigma_\phi^{1/2}u \eqsp,\\
    \nonumber
    &\alpha^{\MALA}_{\phi}(z,u) = 1 \wedge \frac{\pi\bigl(T^{\MALA}_{\phi} (z,u)\bigr) g_\phi\bigl(T^{\MALA}_{\phi} (z, u), z\bigr)} {\pi(z) g_\phi\bigl(z,T^{\MALA}_{\phi} (z, u)\bigr)}  \eqsp,
  \end{align}
  where $g_\phi(z_1,z_2)= |\Sigma_\phi|^{\scriptscriptstyle{-1/2}} \densgauss\bigl(\Sigma_\phi^{\scriptscriptstyle{-1/2}}(z_2-T^{\MALA}_{\phi} (z_1,0))\bigr)$ is the proposal kernel density.



\paragraph{Differentiating through one Markov kernel}
Let $M$ be a Markov kernel, of the form specified above. We wish to derive a reparametrizable expression (in the sense of the reparameterization trick) of a random variable obtained after applying a Markov kernel.
Consider an initial distribution $q$, reparameterizable, and let the Markov kernel $M$ be associated to a proposal mapping family $\{\propmap{u}\colon u\in\msu\}$, a density $\varphi$, and the acceptance function family $\{\alpha_u\colon u\in\msu\}$ -- setting it to 1 recovers the simple transition density case considered above).
Then, a key result is given by the following lemma
\begin{lemma}
\label{lemma:reparam_markov}
  Assume here that the initial distribution has a density, also given by $q$, and that for all $u \in \msu$, $\propmap{u}$ is a $\rmc^1$-diffeomorphism.
  Then, the distribution of the random variable $Z_1$ obtained by drawing $Z_0\sim q$, $Z_1\sim M(Z_0, \cdot)$ has also a density $q_1$, given by
  \begin{multline}
  \label{eq:reparam_markov}
    q_1(z_1 \mid u) = \alpha_u\bigl(\propmap{u}^{-1}(z_1)\bigr) q\bigl(\propmap{u}^{-1}(z_1)\bigr) \Jac_{\propmap{u}^{-1}}(z_1) \\
    + \bigl(1 - \alpha_u(z_1)\bigr) q(z_1)\eqsp,
  \end{multline}
  and we thus have the density $q_1(z_1) = \int_{}q_1(z_1 \mid u) \varphi(u) \rmd u$. 
\end{lemma}
The proof is given in supplementary. Note that if we denote by $a_1$ the output of the A/R procedure, and noting $\alpha_u^1(z) = \alpha_u(z)$, $\alpha^0_u(z) = 1 - \alpha_u(z)$, we can easily define a joint distribution 
\begin{equation}
\label{eq:joint_markov}
  q_1(z_1, a_1, u) = \alpha^{a_1}_u(z) q\bigl(\propmap{u}^{-a_1}(z_1)\bigr) \Jac_{\propmap{u}^{-a_1}}(z_1) \varphi(u) \eqsp.
\end{equation}
%
This expression of course encompasses the case seen above, simply by considering $\alpha_u\equiv 1$:
\begin{equation}
\label{eq:joint_markov_2}
  q_1(z_1, u) =  q\bigl(\propmap{u}^{-1}(z_1)\bigr) \Jac_{\propmap{u}^{-1}}(z_1) \varphi(u) \eqsp.
\end{equation}
%
This distribution is reparameterizable !


\subsection{Differentiable annealed importance sampling estimator}
\label{subsec:ais_estimator}
\begin{comment}
Sequential Importance Sampling (SIS) aims at estimating the normalizing constant $\normconst$ of an unnormalized target density  $\unnormdistr$ on $\rset^{d_z}=\rset^d$.
Suppose we have access to a distribution $\initdistr$ easy to sample from and such that $\initdistr(x) > 0$ whenever $\unnormdistr(x) > 0$.  
A naive importance sampling estimator of $\hat{\normconst}$ is obtained by sampling independently $z^{1},\dots,z^{1}\sim \initdistr$, and compute
\begin{equation}
\label{eq:iS-estimator-Z}
\hat{\normconst} = \frac{1}{n}\sum_{i=1}^n w(z^{i})\eqsp,
\end{equation}
where  $w(x)= \unnormdistr(x)/\initdistr(x)$  is the importance weighting function. % It is well-known that $\hat{\normconst}$ is an unbiased estimator of $Z$ provided . 
However, this estimator might have a very large variance if the importance distribution $\initdistr$ is not chosen carefully.
%In Annealed Importance Sampling (AIS), we rather consider a tempering scheme $(\beta_k)_{k=0}^{K}$, with $0=\beta_0<\beta_1\leq\dots\leq\beta_{K}=1$, and define a sequence of annealed unnormalized target densities $\unnormdistr_k = m^{1-\beta_k} \unnormdistr^{\beta_k }$. With this convention $\unnormdistr_K= \unnormdistr$.

%%Etendre espace, veut que gamma soit la dernière, définit famille de loi copier phrase on etend espace d'etat dans intro
Consider now the path space $\chunk{z}{0}{K}\in \pathspace = \rset^{d{(K+1)}}$an estimator on the extended path space , such that $z_K$ is marginally distributed as the target $\unnormdistr$.
\end{comment}
Recall now the amortized VI problem.
Similarly to \Cref{subsec:sis_est}, 
consider generally two sequences of  Markov  kernels $\{M_{k}\}_{k=1}^K, \{L_{k}\}_{k=0}^{K-1} $, and define on $\pathspace$ the family of distributions
\begin{equation}
  \unnormextendedback(x, \rmd \chunk{z}{0}{K}) = p_\theta(x, \rmd z_K) \prod_{k=K}^1 L_{k-1}(z_{k}, \rmd z_{k-1}) \eqsp.
\end{equation}
%(here $\unnormdistr(\rmd z)$ is a short-hand notation for $\unnormdistr(z) \rmd z$). 
Again, because $\int L_{k-1}(z_{k},\rmd z_{k-1})=1$, the normalizing constant of $\unnormextendedback$ is $\normconst$. 
On the path space, we define an importance distribution
\begin{equation}
    \extendedfor^K(\rmd \chunk{z}{0}{K}\mid x) = \initdistr(\rmd z_0\mid x)\prod_{k=1}^K M_k(z_{k-1},\rmd z_k)\eqsp.
\end{equation}
%which is the distribution of a non-homogeneous Markov chain with initial distribution $\initdistr$ and forward Markov transition $\{M_k\}_{k=1}^K$. 
%Let $\{ \unnormdistr_k \}_{k=0}^K$ be a sequence of unnormalized ``bridge'' distributions satisfying $\unnormdistr_0=\initdistr$ (thus $\unnormdistr_0$ is a probability distribution), $\unnormdistr_K= \unnormdistr$ ($\unnormdistr_K$ is not normalized), with densities also denoted $\{ \unnormdistr_k \}_{k=0}^K$. 
%In all the sequel, we assume that these bridging distributions have densities, also denoted $\{ \unnormdistr_k \}_{k=0}^K$. 
Assume first that there exists a sequence of measurable functions $\{ w_{k,x} \}_{k=0}^{K-1}$ (called importance weights) such that
\begin{multline}
\label{eq:key-assumption}
  \unnormdistr_k(x, \rmd z_k) L_{k-1}(z_k, \rmd z_{k-1}) \\
  = \unnormdistr_{k-1}(x, \rmd z_{k-1}) M_k(z_{k-1}, \rmd z_k) w_{k, x}(z_{k-1},z_k)\eqsp.
\end{multline}
%
We exhibit those weights in the sequel in one particular case of interest. Note that the case presented in \Cref{subsec:sis_est} where we focus on densities is immediate here.
Defining for $k\leq K$ the sequence 
$\unnormextendedbackwithk( x,\rmd \chunk{z}{0}{k}) = \unnormdistr_k(x, \rmd z_k) \prod_{\ell=k}^1 L_{\ell-1}(z_\ell, \rmd z_{\ell-1})$,  note that we can express 
\begin{multline}
  \unnormextendedbackwithk(x,\rmd \chunk{z}{0}{k}) = \unnormextendedbackwithkk(x,\rmd \chunk{z}{0}{k-1})\\ \times w_{k,x}(z_{k-1},z_k) M_k(z_{k-1},\rmd z_k)\eqsp.
\end{multline}
%
Then, since $\unnormdistr_0=\initdistr$, we have
\begin{equation}
\label{eq:key-relation}
  \unnormextendedback(x,\rmd \chunk{z}{0}{K}) = \prod_{k=1}^{K} w_{k,x}(z_{k-1},z_k) \times \extendedfor^K(\rmd \chunk{z}{0}{K}\mid x)\eqsp.
\end{equation}
%
Therefore, the normalizing constant is given by
\begin{multline}
\label{eq:smcsampler_identity}
  \quad\normconst = \int \prod_{k=1}^{K} w_{k,x}(z_{k-1}, z_k) \extendedfor^K(\rmd \chunk{z}{0}{K}\mid x) \eqsp.
\end{multline}
If we can compute the weights $\{w_{k,x}\}_{k=1}^K$, then we have access to an unbiased estimator of $\normconst$ that can be very efficient.
In particular, we might choose the kernels so that $M_k$ is $\unnormdistr_k$-reversible and $L_{k-1} = M_k$, i.e. $\unnormdistr_k(x,\rmd z_k) M_k(z_k,\rmd z_{k-1})=\unnormdistr_{k}(x,\rmd z_{k-1}) M_{k}(z_{k-1},\rmd z_{k})$. Then, we obtain
%For $M_k$ being $\unnormdistr_k$-invariant and $L_{k-1}$ being the corresponding reversal, i.e. $\unnormdistr_k(\rmd z_k) L_{k-1}(z_k,\rmd z_{k-1})=\unnormdistr_{k}(\rmd z_{k-1}) M_{k}(z_{k-1},\rmd z_{k})$, we obtain
\begin{equation}
  \label{eq:weights_ais}
  w_{k,x}(z_{k-1}, z_k) = \frac{\unnormdistr_{k}(x,z_{k-1})}{\unnormdistr_{k-1}(x,z_{k-1})}\eqsp,
\end{equation}
given also by the Jarzynski--Crooks identity~\cite{Jarzynski:1997,crooks1998nonequilibrium} also known as Annealed Importance Sampling identity \cite{neal2001annealed}.
%, see  \Cref{sec:supplementary} for a formal measure-theoretic proof.
Below, we use Metropolis Adjusted Langevin Algorithm (MALA) kernels for AIS. 

\begin{comment}
\paragraph{Using kernel densities: }If  the forward $\{M_k\}_{k=1}^K$ and backward $\{L_k\}_{k=1}^K$ Markov kernels both have positive densities 
%$\{ \unnormdistr_k \}_{k=0}^{K}$, 
$\{ m_k \}_{k=1}^K$, $\{\ell_k\}_{k=0}^{K-1}$, $m_k(z_{k-1},z_k) > 0$ and $\ell_k(z_{k-1},z_k) > 0$, this condition is of course automatically satisfied and the importance weights are then simply defined as
\begin{equation}
\label{eq:weights-smc-density}
w_k(z_{k-1}, z_k) = \frac{\unnormdistr_k(z_k) \ell_{k-1}(z_{k},z_{k-1})}{\unnormdistr_{k-1}(z_{k-1}) m_k(z_{k-1},z_k)} \eqsp.
\end{equation}
In that case, the products of the weights simplifies, and we recognize in that case
\begin{equation}
    \label{eq:prod_weights_with_density}
    \prod_{k=1}^K w_k(z_{k-1}, z_k) = \frac{\unnormdistr_K(z_k)\prod_{k=1}^Kl_{k-1}(z_k, z_{k-1})}{\unnormdistr_{0}(z_{0})\prod_{k=1}^K m_k(z_{k-1}, z_k)}\eqsp.
\end{equation}
This is the general expression that appears for example in Hierarchical Variational Inference (HVI).
Inspired by the similarities drawn with AIS, we might here consider to sample approximately from $\extendedfor$ the Unadjusted Langevin Algorithm (ULA), which shares the same proposal mapping \eqref{eq:langevin_proposal_mapping} as MALA, and has theoretical convergence guarantees. In that case, at each step $k$, we have $M_k(z_{k-1}, \rmd z_k) = \Normal(z_k; z_{k-1} + \stepsize \nabla \log\unnormdistr_k(z_{k-1}), \sqrt{2\stepsize}\Id)$, and if $\densinnovation$ is the density of the innovation noise, standard normal Gaussian here, then $m_k(z_{k-1}, z_k) = \densinnovation((z_k - z_{k-1} - \stepsize \nabla \log\unnormdistr_k(z_{k-1}))/\sqrt{2\stepsize}) \sqrt{2\stepsize}^d$. We choose as well $L_{k-1} = M_k$.
%, in which $\prod_{k=1}^Kl_{k-1}(z_k, z_{k-1})$ are the ``reverse kernels'' that we usually want to find and optimize.
\paragraph{Using deterministic kernels: }Assume now that the forward kernels $\{ M_k \}_{k=0}^{K-1}$ are deterministic: $M_k(z_{k-1},\rmd z_k)= \delta_{\propmap{k}(z_{k-1})}(\rmd z_k)$ where $\propmap{k}$ is a diffeomorphism on $\rset^{d_z}$. 
Then \eqref{eq:key-assumption} holds with $L_{k-1}(z_k, \rmd z_{k-1})= \delta_{\propmap{k}^{-1}(z_k)}(\rmd z_{k-1})$ if we set 
\begin{equation}
\label{eq:weight-deterministic}
w_k(z_{k-1},z_k)=  \frac{\unnormdistr_k(\propmap{k}(z_{k-1}) \Jac_{\propmap{k}}(z_{k-1}))}{\unnormdistr_{k-1}(z_{k-1})} \indi{\propmap{k}(z_{k-1})}(z_k) \eqsp.
\end{equation}
In such case, the product $\prod_{k=1}^K w_k(z_{k-1},z_k)$ is given, for $z_k= \propmap{k}(z_{k-1})$, $k=1,\dots,K$, by 
\begin{equation}
\label{eq:product-weight-deterministic}
\prod_{k=1}^K w_k(z_{k-1},z_k) = \frac{\unnormdistr_K(z_K)}{\unnormdistr_0(z_0)} \prod_{k=1}^K \Jac_{\propmap{k}}(z_{k-1}) \eqsp.
\end{equation}
We retrieve here the ``plain" important sampling estimator. We can also draw some attention to the reader between this formulation and the Continously Indexed Flows framework, presented in \cite{cornish:caterini:doucet:2020}, see Supplementary. This will however not be our main interest in the sequel, as we will focus on the cases presented before.
%Hence if  $\{\chunk{z^{(i)}}{0}{K}\}_{i=1}^n$ are $n$ independent trajectories from $\extendedfor$, then
%\begin{equation}
%    \hat{\normconst} = \frac{1}{n} \sum_{i=1}^n \left[  \prod_{k=1}^{K}  w_k(z^{(i)}_{k-1}, z^{(i)}_k)\right]\eqsp,
%\end{equation}
%is an unbiased estimator of $\normconst$. This is known as the sequential importance sampling estimator in ML. Note that if $K=0$, we recognize the usual importance sampling estimator.
\end{comment}
We would like to rely on those estimators to perform Variational Inference to learn parameters $\phi$ of the initial distribution $\initdistr$ and of parameters $\theta$ of the target distribution.

\paragraph{Writing the reparameterization trick with conditional kernels}
  The idea is to build on the expression of the estimators and the kernels written in \cite{thin:2020} fashion to derive an ELBO with SIS that is differentiable and has by design a nice expression.

  For simplicity of notation, we consider here the cases where $L_{k-1} = M_{k}$ for $k\leq K$. Note that we could easily generalize to other cases, especially inspired by recent works on non-reversibility of MCMC procedures~\cite{thin:kotelevskii:andrieu:moulines:2020}.
  By the AIS estimator, we are given, for $1 \leq k \leq K$, kernels $\{M_{k}\}_{k=1}^K, %\{L_{k}\}_{k=0}^{K-1} 
  $ associated to the conditional kernel for $u\in\msu$, $Q_{k,u}$ and the density of the innovation noise $\densinnovation$, the proposal mappings $\propmap{k,u}$ and the acceptance functions $\alpha_{k,u}$ if we consider reversible Markov kernels, \ie~the AIS estimator.
%  Note that again, we write these acceptance functions in the following for generality's sake, however, when considering kernel densities, we choose these acceptance function to be identically equal to 1.

  By definition of the extended distribution $\extendedfor^K$, we have
  \begin{equation}
    \extendedfor^K(\rmd \chunk{z}{0}{K}| x) =  \initdistr(\rmd z_0| x)  \int_{} \prod_{t=1}^K Q_{t,u_t}(z_{t-1},\rmd z_t) \densinnovation(\chunk{u}{1}{K})\rmd\chunk{u}{1}{K} \eqsp,
  \end{equation}
  where we write by an abuse of notation $\densinnovation(\chunk{u}{1}{K})= \prod_{t=1}^K \densinnovation(u_t)$.
  Note now, for $1\leq t\leq K, u\in\msu$, $\alpha^1_{t, u_t} \equiv \alpha_{t, u_t}$ and $\alpha^0_{t, u_t}\equiv 1-\alpha_{t, u_t}$, and for transformations $\{T_j\}_{j=i}^K$, $\Circ{j=i}{K} = T_K\circ\dots\circ T_i$. Write by convention as well for a transformation $T$, $T^1 = T$ and $T^0 = \Id$.
  By \Cref{lemma:reparam_markov}, we can define as well the extended distribution
  \begin{multline}
    \extendedfor^K({\rmd \chunk{z}{0}{K}, \chunk{a}{1}{K},\rmd \chunk{u}{1}{K}}\mid x) = \\
    \initdistr(\rmd z_0\mid x) \prod_{t=1}^K \alpha^{a_t}_{t, u_t} \bigl( z_{t-1}\bigr)  \updelta_{\propmap{t, u_{t}}^{a_t}(z_{t-1})}(\rmd z_t)\densinnovation(\chunk{u}{1}{K})\rmd\chunk{u}{1}{K} \eqsp.
  \end{multline}
  By~\eqref{eq:smcsampler_identity}, we have using Jensen's inequality and the previous representation of Metropolis Hastings kernels, we can  write
  {\small\begin{align}
    &\log \normconst = \log\hspace{-5pt} \int_{} \sum_{\chunk{a}{1}{K}}  \extendedfor^K({\rmd \chunk{z}{0}{K}, \chunk{a}{1}{K},\rmd \chunk{u}{1}{K}}|x) \prod_{k = 1}^{K}  w_{k,x}(z_{t-1}, z_t) \\
    &\geq  \int \sum_{\chunk{a}{1}{K}}  \extendedfor^K({\rmd \chunk{z}{0}{K}, \chunk{a}{1}{K},\rmd \chunk{u}{1}{K}}|x) \log\left(\prod_{k = 1}^{K}  w_{k,x}(z_{t-1}, z_t)\right) \\
    %&\geq   \int \sum_{\chunk{a}{1}{K}}  \initdistr( z_0) \prod_{t=1}^K \alpha^{a_t}_{t,u_t} \bigl( z_{t-1}\bigr) \densinnovation( \chunk{u}{1}{K})  \updelta_{\propmap{t, u_{t}}^{a_t}(z_{t-1})}(\rmd z_t) \log\left( \prod_{t=1}^{K}  w_t(z_{t-1}, z_t)\right)\rmd z_0\rmd \chunk{u}{1}{K}\\
    &\geq \int \sum_{\chunk{a}{1}{K}}  \initdistr( z_0|x) \prod_{t=1}^K \alpha^{a_t}_{t,u_t} \bigl(\Circ{i=1}{t-1} \propmap{i, u_i}^{a_i} (z_0)\bigr) \densinnovation(\chunk{u}{1}{K}) \\
    &\quad\times\log\left(\prod_{k = 1}^{K} w_{k,x}\Bigl(\Circ{i = 1}{t-1} \propmap{i, u_i}^{a_i} (z_0), \Circ{i = 1}{t} \propmap{i, u_i}^{a_i} (z_0)\Bigr)\right) \rmd z_0\rmd \chunk{u}{1}{K}\eqsp,
  \end{align}}
  where in the last line we have integrated \wrt~$z_K, z_{K-1}, \dots, z_1$.
  This expression is now differentiable by the reparameterization trick, and we can optimize \wrt~the different parameters at stake (even possibly the parameters of the proposal mappings).
  Note however that the discrete distribution over the $\chunk{a}{1}{K}$ is not directly reparametrizable, and we thus have to resort to a score function expression of the gradient over this quantity. The precise expression is given in Supplementary, due to lack of space here. An extension of our work would implement the Concrete distribution and the Gumbel Softmax trick \cite{maddison2016concrete} to write another version of the gradient.
  %Moreover, thanks to the expression of the AIS estimator, even though we are performing MH steps, we are exactly optimizing an estimator (and a close one) to the normalizing constant, contrarily to \cite{thin:2020}.
  The algorithm to estimate the differentiable AIS estimator is given in \Cref{alg:differentiable_ais}.
 \begin{algorithm}[!ht]
    \caption{Differentiable Langevin Sequential Importance Sampling }
    \label{alg:differentiable_sis_flows}
    \begin{algorithmic}
      \STATE {\bfseries Input:}  Number of steps $K$, proposal mappings $\{\propmap{t, u}\}_{t \leq K, u\in\msu}$, initial distribution $\initdistr$, unnormalized target distribution $p_\theta$, densities $\{m_{t}\}_{t = 1}^K, \{l_{t}\}_{t = 0}^{K - 1} $.
       \STATE {\bfseries Output:} SIS estimator of the log normalizing constant $S_w$.
        \\\hrulefill
        \STATE Draw $z_0\sim \initdistr(\cdot\mid x)$;
        \STATE Set $S_w = -\log \initdistr(z_0\mid x)$;
      \FOR{$t=1$ {\bfseries to} $K$}
      \STATE Draw $u_t\sim \densinnovation$;
      \STATE Set $z_t = \propmap{t, u_t}(z_{t - 1})$;
      \STATE Set $S_w = S_w + \log l_{t - 1}(z_{t}, z_{t - 1}) - \log m_t(z_{t - 1}, z_t)$;
      \ENDFOR
      \STATE Set $S_w = S_w + \log p_\theta (x,z_K)$;
      \STATE Return $S_w$
    \end{algorithmic}
  \end{algorithm}
  \begin{algorithm}[!ht]
    \caption{Differentiable Annealed Importance Sampling}
    \label{alg:differentiable_ais}
    \begin{algorithmic}
      \STATE {\bfseries Input:}  Number of steps $K$, proposal mappings $\{\propmap{t, u}\}_{t\leq K, u\in\msu}$, acceptance function $\{\alpha_{t,u}\}_{t\leq K, u\in\msu}$, initial distribution $\initdistr$, unnormalized target distribution $p_\theta$, annealing schedule $\{\beta_t\}_{t=0}^{K}$.
       \STATE {\bfseries Output:} AIS estimator of the log normalizing constant $S_w$, sum $S_\alpha$ of the A/R log probabilities.
        \\\hrulefill
        \STATE Draw $z_0\sim \initdistr(\cdot\mid x)$;
        \STATE Set $S_w = 0$;%\log w_0(z_0) = (\beta_1 -\beta_0) (\log\unnormdistr(z_0) -\log \initdistr(z_0))$;
        \STATE Set $S_\alpha = 0$;
      \FOR{$t=1$ {\bfseries to} $K$}
      \STATE Draw $u_t\sim \densinnovation$;
      \STATE Draw $a_t \sim \Ber(\alpha_{t,u_t}\bigl(z_{t - 1})\bigr)$;
      \STATE Set $z_t = \propmap{t, u_t}^{a_t}(z_{t - 1})$;
      \STATE Compute $\log w_{t,x}(z_{t - 1}, z_t) =$ \\
      \qquad$(\beta_{t} -\beta_{t-1})\left(\log p_\theta(x, z_{t - 1}) - \log\initdistr(z_{t - 1}\mid x)\right)$;
      \STATE Set $S_w = S_w + \log w_{t,x}(z_{t - 1}, z_t)$ ;
      \STATE Set $S_\alpha = S_\alpha + \log \alpha^{a_t}_{t,u_t}(z_{t-1})$;
      \ENDFOR
      \STATE Return $S_w, S_\alpha$
    \end{algorithmic}
  \end{algorithm}
% Note the particular objectives considered in \cite{huang:tan:lacoste:courville:2018} consider each of the incremental weights in the non reversible case with kernel densities, that is \[\log w_k(z_{k-1}, z_k) = \log \frac{\unnormdistr_k (z_k) l_{k-1}(z_{k}, z_{k-1})}{ \unnormdistr_{k-1}(z_{k-1}) m_k(z_{k-1}, z_k)}\eqsp,\]and attempt at maximizing each of them individually.

==> related_work.tex <==
% !TEX root = main.tex

TODO

==> smc.tex <==
% !TEX root = main.tex

\subsection{Differentiable annealed importance sampling estimator}
\label{subsec:ais_estimator}
\begin{comment}
Sequential Importance Sampling (SIS) aims at estimating the normalizing constant $\normconst$ of an unnormalized target density  $\unnormdistr$ on $\rset^{d_z}=\rset^d$.
Suppose we have access to a distribution $\initdistr$ easy to sample from and such that $\initdistr(x) > 0$ whenever $\unnormdistr(x) > 0$.  
A naive importance sampling estimator of $\hat{\normconst}$ is obtained by sampling independently $z^{1},\dots,z^{1}\sim \initdistr$, and compute
\begin{equation}
\label{eq:iS-estimator-Z}
\hat{\normconst} = \frac{1}{n}\sum_{i=1}^n w(z^{i})\eqsp,
\end{equation}
where  $w(x)= \unnormdistr(x)/\initdistr(x)$  is the importance weighting function. % It is well-known that $\hat{\normconst}$ is an unbiased estimator of $Z$ provided . 
However, this estimator might have a very large variance if the importance distribution $\initdistr$ is not chosen carefully.
%In Annealed Importance Sampling (AIS), we rather consider a tempering scheme $(\beta_k)_{k=0}^{K}$, with $0=\beta_0<\beta_1\leq\dots\leq\beta_{K}=1$, and define a sequence of annealed unnormalized target densities $\unnormdistr_k = m^{1-\beta_k} \unnormdistr^{\beta_k }$. With this convention $\unnormdistr_K= \unnormdistr$.

%%Etendre espace, veut que gamma soit la dernière, définit famille de loi copier phrase on etend espace d'etat dans intro
Consider now the path space $\chunk{z}{0}{K}\in \pathspace = \rset^{d{(K+1)}}$an estimator on the extended path space , such that $z_K$ is marginally distributed as the target $\unnormdistr$.
\end{comment}
Recall now the amortized VI problem.
Similarly to \Cref{subsec:sis_est}, 
consider generally two sequences of  Markov  kernels $\{M_{k}\}_{k=1}^K, \{L_{k}\}_{k=0}^{K-1} $, and define on $\pathspace$ the family of distributions
\begin{equation}
    \unnormextendedback(x, \rmd \chunk{z}{0}{K}) = p_\theta(x, \rmd z_K) \prod_{k=K}^1 L_{k-1}(z_{k}, \rmd z_{k-1}) \eqsp.
\end{equation}
%(here $\unnormdistr(\rmd z)$ is a short-hand notation for $\unnormdistr(z) \rmd z$). 
Again, because $\int L_{k-1}(z_{k},\rmd z_{k-1})=1$, the normalizing constant of $\unnormextendedback$ is $\normconst$. 
On the path space, we define an importance distribution
\begin{equation}
  \extendedfor^K(\rmd \chunk{z}{0}{K}\mid x) = \initdistr(\rmd z_0\mid x)\prod_{k=1}^K M_k(z_{k-1},\rmd z_k)\eqsp.
\end{equation}
%which is the distribution of a non-homogeneous Markov chain with initial distribution $\initdistr$ and forward Markov transition $\{M_k\}_{k=1}^K$. 
%Let $\{ \unnormdistr_k \}_{k=0}^K$ be a sequence of unnormalized ``bridge'' distributions satisfying $\unnormdistr_0=\initdistr$ (thus $\unnormdistr_0$ is a probability distribution), $\unnormdistr_K= \unnormdistr$ ($\unnormdistr_K$ is not normalized), with densities also denoted $\{ \unnormdistr_k \}_{k=0}^K$. 
%In all the sequel, we assume that these bridging distributions have densities, also denoted $\{ \unnormdistr_k \}_{k=0}^K$. 
Assume first that there exists a sequence of measurable functions $\{ w_{k,x} \}_{k=0}^{K-1}$ (called importance weights) such that
\begin{multline}
\label{eq:key-assumption}
  \unnormdistr_k(x, \rmd z_k) L_{k-1}(z_k, \rmd z_{k-1})=\\ \unnormdistr_{k-1}(x, \rmd z_{k-1}) M_k(z_{k-1}, \rmd z_k) w_{k, x}(z_{k-1},z_k)\eqsp.
\end{multline}
%
We exhibit those weights in the sequel in one particular case of interest. Note that the case presented in \Cref{subsec:sis_est} where we focus on densities is immediate here.
Defining for $k\leq K$ the sequence 
$\unnormextendedbackwithk( x,\rmd \chunk{z}{0}{k})= \unnormdistr_k(x, \rmd z_k) \prod_{\ell=k}^1 L_{\ell-1}(z_\ell, \rmd z_{\ell-1})$,  note that we can express 
\begin{multline}
  \unnormextendedbackwithk(x,\rmd \chunk{z}{0}{k})= \unnormextendedbackwithkk(x,\rmd \chunk{z}{0}{k-1})\\ \times w_{k,x}(z_{k-1},z_k) M_k(z_{k-1},\rmd z_k)\eqsp.
\end{multline}
%
Then, since $\unnormdistr_0=\initdistr$, we have
\begin{equation}
\label{eq:key-relation}
  \unnormextendedback(x,\rmd \chunk{z}{0}{K}) = \prod_{k=1}^{K} w_{k,x}(z_{k-1},z_k) \times \extendedfor^K(\rmd \chunk{z}{0}{K}\mid x)\eqsp.
\end{equation}
%
Therefore, the normalizing constant is given by
\begin{multline}
\label{eq:smcsampler_identity}
  \quad\normconst = \int \prod_{k=1}^{K} w_{k,x}(z_{k-1}, z_k) \extendedfor^K(\rmd \chunk{z}{0}{K}\mid x) \eqsp.
\end{multline}
%
If we can compute the weights $\{w_{k,x}\}_{k=1}^K$, then we have access to an unbiased estimator of $\normconst$ that can be very efficient.
In particular, we might choose the kernels so that $M_k$ is $\unnormdistr_k$-reversible and $L_{k-1} = M_k$, i.e. $\unnormdistr_k(x,\rmd z_k) M_k(z_k,\rmd z_{k-1})=\unnormdistr_{k}(x,\rmd z_{k-1}) M_{k}(z_{k-1},\rmd z_{k})$. Then, we obtain
%For $M_k$ being $\unnormdistr_k$-invariant and $L_{k-1}$ being the corresponding reversal, i.e. $\unnormdistr_k(\rmd z_k) L_{k-1}(z_k,\rmd z_{k-1})=\unnormdistr_{k}(\rmd z_{k-1}) M_{k}(z_{k-1},\rmd z_{k})$, we obtain
\begin{equation}
  \label{eq:weights_ais}
  \qquad w_{k,x}(z_{k-1}, z_k) = \frac{\unnormdistr_{k}(x,z_{k-1})}{\unnormdistr_{k-1}(x,z_{k-1})}\eqsp,
\end{equation}
given also by the Jarzynski--Crooks identity~\cite{Jarzynski:1997,crooks1998nonequilibrium} also known as Annealed Importance Sampling identity~\cite{neal2001annealed}.
%, see  \Cref{sec:supplementary} for a formal measure-theoretic proof.
Below, we use Metropolis Adjusted Langevin Algorithm (MALA) kernels for AIS. 

\begin{comment}
\paragraph{Using kernel densities: }If  the forward $\{M_k\}_{k=1}^K$ and backward $\{L_k\}_{k=1}^K$ Markov kernels both have positive densities 
%$\{ \unnormdistr_k \}_{k=0}^{K}$, 
$\{ m_k \}_{k=1}^K$, $\{\ell_k\}_{k=0}^{K-1}$, $m_k(z_{k-1},z_k) > 0$ and $\ell_k(z_{k-1},z_k) > 0$, this condition is of course automatically satisfied and the importance weights are then simply defined as
\begin{equation}
\label{eq:weights-smc-density}
w_k(z_{k-1}, z_k) = \frac{\unnormdistr_k(z_k) \ell_{k-1}(z_{k},z_{k-1})}{\unnormdistr_{k-1}(z_{k-1}) m_k(z_{k-1},z_k)} \eqsp.
\end{equation}
In that case, the products of the weights simplifies, and we recognize in that case
\begin{equation}
    \label{eq:prod_weights_with_density}
    \prod_{k=1}^K w_k(z_{k-1}, z_k) = \frac{\unnormdistr_K(z_k)\prod_{k=1}^Kl_{k-1}(z_k, z_{k-1})}{\unnormdistr_{0}(z_{0})\prod_{k=1}^K m_k(z_{k-1}, z_k)}\eqsp.
\end{equation}
This is the general expression that appears for example in Hierarchical Variational Inference (HVI).
Inspired by the similarities drawn with AIS, we might here consider to sample approximately from $\extendedfor$ the Unadjusted Langevin Algorithm (ULA), which shares the same proposal mapping \eqref{eq:langevin_proposal_mapping} as MALA, and has theoretical convergence guarantees. In that case, at each step $k$, we have $M_k(z_{k-1}, \rmd z_k) = \Normal(z_k; z_{k-1} + \stepsize \nabla \log\unnormdistr_k(z_{k-1}), \sqrt{2\stepsize}\Id)$, and if $\densinnovation$ is the density of the innovation noise, standard normal Gaussian here, then $m_k(z_{k-1}, z_k) = \densinnovation((z_k - z_{k-1} - \stepsize \nabla \log\unnormdistr_k(z_{k-1}))/\sqrt{2\stepsize}) \sqrt{2\stepsize}^d$. We choose as well $L_{k-1} = M_k$.
%, in which $\prod_{k=1}^Kl_{k-1}(z_k, z_{k-1})$ are the ``reverse kernels'' that we usually want to find and optimize.
\paragraph{Using deterministic kernels: }Assume now that the forward kernels $\{ M_k \}_{k=0}^{K-1}$ are deterministic: $M_k(z_{k-1},\rmd z_k)= \delta_{\propmap{k}(z_{k-1})}(\rmd z_k)$ where $\propmap{k}$ is a diffeomorphism on $\rset^{d_z}$. 
Then \eqref{eq:key-assumption} holds with $L_{k-1}(z_k, \rmd z_{k-1})= \delta_{\propmap{k}^{-1}(z_k)}(\rmd z_{k-1})$ if we set 
\begin{equation}
\label{eq:weight-deterministic}
w_k(z_{k-1},z_k)=  \frac{\unnormdistr_k(\propmap{k}(z_{k-1}) \Jac_{\propmap{k}}(z_{k-1}))}{\unnormdistr_{k-1}(z_{k-1})} \indi{\propmap{k}(z_{k-1})}(z_k) \eqsp.
\end{equation}
In such case, the product $\prod_{k=1}^K w_k(z_{k-1},z_k)$ is given, for $z_k= \propmap{k}(z_{k-1})$, $k=1,\dots,K$, by 
\begin{equation}
\label{eq:product-weight-deterministic}
\prod_{k=1}^K w_k(z_{k-1},z_k) = \frac{\unnormdistr_K(z_K)}{\unnormdistr_0(z_0)} \prod_{k=1}^K \Jac_{\propmap{k}}(z_{k-1}) \eqsp.
\end{equation}
We retrieve here the ``plain" important sampling estimator. We can also draw some attention to the reader between this formulation and the Continously Indexed Flows framework, presented in \cite{cornish:caterini:doucet:2020}, see Supplementary. This will however not be our main interest in the sequel, as we will focus on the cases presented before.
%Hence if  $\{\chunk{z^{(i)}}{0}{K}\}_{i=1}^n$ are $n$ independent trajectories from $\extendedfor$, then
%\begin{equation}
%    \hat{\normconst} = \frac{1}{n} \sum_{i=1}^n \left[  \prod_{k=1}^{K}  w_k(z^{(i)}_{k-1}, z^{(i)}_k)\right]\eqsp,
%\end{equation}
%is an unbiased estimator of $\normconst$. This is known as the sequential importance sampling estimator in ML. Note that if $K=0$, we recognize the usual importance sampling estimator.
\end{comment}
We would like to rely on those estimators to perform Variational Inference to learn parameters $\phi$ of the initial distribution $\initdistr$ and of parameters $\theta$ of the target distribution.


==> smc_density.tex <==
% !TEX root = main.tex


%We focus in the following on deriving efficient and differentiable estimators of the likelihood $p_\theta(x)$, based in particular on Sequential Monte Carlo ideas.

\subsection{Sequential importance sampling estimator}
%Sequential Importance Sampling (SIS) aims at estimating the normalizing constant $\normconst$ of an unnormalized target density  $\unnormdistr$ on $\rset^{d_z}=\rset^d$.
%Suppose we have access to a distribution $\initdistr$ easy to sample from and such that $\initdistr(z) > 0$ whenever $\unnormdistr(z) > 0$.  
\label{subsec:sis_est}
A importance sampling estimator of $\hatnormconst$ is obtained by sampling independently $z^{1}, \dots, z^{n} \sim \initdistr(\cdot\mid x)$, and compute
\begin{equation}
\label{eq:iS-estimator-Z}
\hatnormconst = \frac{1}{n}\sum_{i=1}^n w(z^{i})\eqsp,
\end{equation}
where  $w(z)= p_\theta(x,z)/\initdistr(z\mid x)$  is the importance weighting function. % It is well-known that $\hatnormconst$ is an unbiased estimator of $Z$ provided . 
This is the core idea of the IWAE.
However, in general in importance sampling, this estimator might have a very large variance if the importance distribution $\initdistr$ is not chosen carefully.
%In Annealed Importance Sampling (AIS), we rather consider a tempering scheme $(\beta_k)_{k=0}^{K}$, with $0=\beta_0<\beta_1\leq\dots\leq\beta_{K}=1$, and define a sequence of annealed unnormalized target densities $\unnormdistr_k = m^{1-\beta_k} \unnormdistr^{\beta_k }$. With this convention $\unnormdistr_K= \unnormdistr$.

%%Etendre espace, veut que gamma soit la dernière, définit famille de loi copier phrase on etend espace d'etat dans intro

To introduce a good proposal importance distribution, it has been suggested in the literature \cite{neal2001annealed} to use temperature tempering, or annealing: let $\{\unnormdistr_k\}_{k=0}^K$ be a sequence of unnormalized ``bridge'' densities satisfying $\unnormdistr_0(x, \cdot) = \initdistr(\cdot\mid x)$ (thus $\unnormdistr_0$ is a probability density), $\unnormdistr_K(\cdot, x)= p_\theta(x, \cdot)$ ($\unnormdistr_K$ is not normalized).
Consider then a sequence of positive transition densities $\{ m_k \}_{k=1}^K$. 
In spirit, $m_k$ leaves $\unnormdistr_k$ invariant, meaning that we take advantage of the transition densities to ``transport'' initial samples from $\initdistr = \unnormdistr_0$ to $p_\theta = \unnormdistr_K$. Typically, $m_k$ depends on the data $x$. However, by simplicity of notation, we now omit $x$ in the transition densities.
The idea is to build from those transitions a path space that will transport original samples from $\initdistr$ to $p_\theta$. \achille{two sentence proposals here, choose only one sentence}
Define the extended proposal distribution
\begin{equation}
  \initdistr^K(\chunk{z}{0}{K} \mid x) = \initdistr(z_0 \mid x) \prod_{k=1}^K m_k(z_{k-1}, z_k)\eqsp,
\end{equation}
where $\chunk{z}{i}{j} = (z_i, \dots, z_j)$ for $0 \leq i \leq j$.
In order to perform directly importance sampling, one would need access to the $K$-th marginal of this pdf $\initdistr^K(z_K\mid x)$. 
However, this quantity is typically not tractable. 
Then, to perform properly SIS, we usually then introduce another sequence of normalized positive transition densities $\{\ell_k\}_{k = 0}^{K-1}$.
We then consider the path space $\chunk{z}{0}{K} \in \rset^{d{(K + 1)}}$, and define the extended target density
\begin{equation}
  p_\theta^K(x, \chunk{z}{0}{K}) = p_\theta(x, z_K) \prod_{k=K-1}^0 \ell_{k}(z_{k+1},z_{k})\eqsp.
\end{equation}
%
By construction, we have that $\int p_\theta^K(x, \chunk{z}{0}{K}) \rmd \chunk{z}{0}{K-1} = p_\theta(x, z_K)$, which means that $z_K$ is marginally distributed as the target $p_\theta$. 
Moreover, as the transition densities are normalized, we have $\int p_\theta^K(x, \chunk{z}{0}{K}) \rmd \chunk{z}{0}{K} = \normconst$. 

This defines a sequence of importance weights $\{w_{k, x}\}_{k = 1}^{K}$ such that 
\begin{equation}
  w_{k,x}(z_{k-1}, z_k) = \frac{\unnormdistr_k(x, z_k) \ell_{k-1}(z_{k}, z_{k-1})}{\unnormdistr_{k-1}(x, z_{k-1}) m_k(z_{k-1}, z_k)} \eqsp.
\end{equation}
Then, finally, the unbiased estimator given by SIS and proposed in~\cite{Del-Moral:2006,salimans:kingma:welling:2015} is in this case
\begin{multline}
\label{eq:SiS-estimator-Z}
  \hatnormconst = \frac{1}{n}\sum_{i = 1}^n \prod_{k = 1}^K w_{k, x} (z_{k-1}^{i}, z_k^i), \, \chunk{z}{0}{K}^i \sim \initdistr^K(\cdot | x).
\end{multline}
%
We detail now our choice for the transition densities. A key feature is that ideally, for each $k$, $m_k$ is invariant \wrt the density $\unnormdistr_k$ to ensure that the marginal distribution of $Z_K$ under $\initdistr^K$ is close to $p_\theta$. The optimal reverse kernels $\ell_k$ minimizing the variance of $\hatnormconst$ are given in~\cite{Del-Moral:2006} by 
\begin{multline}
\label{eq:optimalbackward}
  \ell_{k-1}(z_k,z_{k-1})=\frac{q_{\phi,k-1}(z_{k-1})m_k(z_{k-1}, z_k)}{q_{\phi,k}(z_k)}\eqsp,
\end{multline}
where $q_{\phi,k}$ is the marginal density of $Z_k$ under $\initdistr^K$. However, this leads to $\hatnormconst=\unnormdistr_k(z_K)/q_K(z_K)$ which is intractable. In~\cite{salimans:kingma:welling:2015}, it has been proposed to parameterize a neural network for the densities $l_k$ to be learnt. This introduces flexibility in the model, but can be quite computationally expensive. This has also generally been considered in~\cite{huang:tan:lacoste:courville:2018}, but again, the transitions are heavily parameterized. However, the expression~\eqref{eq:optimalbackward} suggest various approximations of $\ell_{k-1}$. In particular if we assume $q_{\phi,k} \approx q_{\phi,k-1} \approx \gamma_k$, then $\ell_{k-1}$ is the reversal of $m_k$ used by AIS~\cite{crooks1998nonequilibrium,neal2001annealed}. 


\subsection{Sequential importance sampling meets Langevin}
On the other hand, assume now that the target distribution $p_\theta$ is continuously differentiable. Then, the Langevin dynamics associated with the target distribution $p_\theta$ defines a stochastic differential equation \cite{} which is reversible \wrt $p_\theta$ and leaves it invariant. 
A usual way to construct an efficient sampling scheme based on this Langevin dynamics is to consider the Euler-Maruyama discretization of the dynamics, which defines the chain $\{Z_k\}_{k\in\nset}$ recursively with
\begin{equation}
  Z_{k} = Z_{k-1} + \stepsize \nabla\log\unnormdistr_k(Z_{k-1}) + \sqrt{2\stepsize} U_{k}\eqsp,
\end{equation}
where $U_{k+1} \sim \varphi$, where $\varphi$ denotes the density of the $d$ dimensional standard normal distribution. 
Inspired by Langevin dynamics, we consider the transition density $m_k$ associated with one step of Langevin, that is
$m_k(z_{k-1}, z_k) = \Normal(z_k; z_{k-1} + \stepsize\nabla\log\unnormdistr_k(z_{k-1}),2\stepsize \Id )$. Moreover, as the continuous Langevin dynamics is reversible \wrt\ $\unnormdistr_k$, then we can approximate the optimal $l_{k-1}$ by $m_k$ directly.\textcolor{red}{refer to the reversal expression to justify it}

Finally, we would like to be able to reparameterize the final sample $z_K$. We define the Langevin mappings, for $k\in\{1,\dots, K\}$, 
\begin{equation}
  \propmap{k, u}(z_{k-1}) = z_{k-1} + \stepsize\nabla\log\unnormdistr_k(z_{k-1}) + \sqrt{2\stepsize} u\eqsp.
\end{equation}
%
We can consider the noise Langevin mapping similarly, $G_{k, z_{k-1}}\colon u \mapsto z_{k-1} + \stepsize\nabla\log\unnormdistr_k(z_{k-1}) + \sqrt{2\stepsize} u $, which is obviously a diffeomorphism. Such representation allows us to write the density $m_k(z_{k-1}, z_k)= \Jac_{G^{-1}_{k, z_{k-1}}}(z_k) \varphi\bigl(G^{-1}_{k, z_{k-1}}(z_k)\bigr)$ with a simple computation. This will be useful to reparameterize our final objective.
Drawing from $\initdistr^K$ is straightforward and goes as follows:
(i) Draw $z_0\sim \initdistr(\cdot\mid x)$, (ii) For $k = 1:K$, draw $z_k \sim m(z_{k-1})$, \ie\ draw $u_k \sim \varphi$, set $z_k = \propmap{k, u_k}(z_{k-1})$.
Note, for transformations $\{T_j\}_{j=i}^K$, $\Circ{j=i}{K} = T_K \circ \dots \circ T_i$. Write by convention as well for a transformation $T$, $T^1 = T$ and $T^0 = \Id$.
By~\eqref{eq:SiS-estimator-Z}, we have 
%{\small
\begin{align}
  \label{eq:elbo_sis}
  \nonumber &\log \normconst = \log \int \prod_{k=1}^K w_{k,x} (z_{k-1}, z_k) \initdistr^K(\chunk{z}{0}{K}\mid x) \rmd \chunk{z}{0}{K} \\
  \nonumber &\geq  \int \log \left(\prod_{k=1}^K w_{k,x} (z_{k-1}, z_k)\right) \initdistr^K(\chunk{z}{0}{K}\mid x) \rmd \chunk{z}{0}{K}\\
  &\geq  \int \log\left( \prod_{k=1}^{K}  w_{k,x}(z_{k-1},z_k)\right)\initdistr(z_0\mid x) \varphi(\chunk{u}{1}{K})\rmd z_0\rmd \chunk{u}{1}{K},
\end{align}
%}
where we have noted by abuse of notation $\varphi(\chunk{u}{1}{K}) = \prod_{i=1}^K \varphi(u_i)$ and for all $k$, $z_k = \Circ{i=1}{k} \propmap{i, u_i} (z_0)$.
The proof of last line is given in supplementary, but we give here a flavour of the proof in the case $K=1$, and where we consider Langevin transitions.
\begin{align}
\nonumber
  &\int \log \bigl(w_{1, x} (z_{0}, z_1)\bigr) \initdistr^1(\chunk{z}{0}{1}\mid x) \rmd \chunk{z}{0}{1} \\
  &= \int \log \bigl(w_{1, x} (z_{0}, z_1)\bigr) \initdistr(z_0\mid x)\Jac_{G^{-1}_{1, z_{0}}}(z_1) \varphi\bigl(G^{-1}_{1, z_{0}}(z_1)\bigr)  \rmd \chunk{z}{0}{1}\\
  &= \int \log \bigl(w_{1, x} (z_{0}, \propmap{1, u_1}(z_0))\bigr) \initdistr(z_0 \mid x) \varphi(u_1) \rmd z_0 \rmd u_1\eqsp,
\end{align}
and at the last line, we have performed the change of variables $u_1 = G^{-1}_{1, z_{0}}(z_1)$, hence $z_1 = G_{1, z_{0}}(u_1) = \propmap{1, u_1}(z_0)$ by definition. 

Our objective thus finally becomes
\begin{multline}
  \elbosmc(\theta, \phi; x) = \int q_\phi(z_0\mid x) \densinnovation(\chunk{u}{1}{K}) \\
  \log\left(\frac{p_\theta(x, z_K)\prod_{k=1}^K l_{k-1}(z_k, z_{k-1})}{q_\phi(z_0 \mid x) \prod_{k = 1}^K m_k(z_{k-1}, z_k)}\right) \rmd z_0 \rmd \chunk{u}{1}{K}\eqsp,
\end{multline}
This defines a differentiable Annealed Langevin Variational Inference algorithm, described in \Cref{alg:differentiable_sis_flows}. Note that this type of flow can also be related to the one presented in~\cite{caterini:doucet:2018}, however the authors in this work do not consider a randomization by adding additional innovation noise at each step.

One drawback of this approach is that we only consider approximately reversible kernels (due to the discretization error of the Langevin equation, in particular here).
In order to satisfy reversibility for the Langevin dynamics, one must introduce a Metropolis Hastings correction step.
However, this correction step implies that the resulting Markov kernel does not have a density. We propose in the next section a representation which allows us to differentiate through a Markov kernel, even with a Metropolis Hastings step. However, we need however to rely a little bit on measure theoretical notations in order to ensure the validity of our approach. Those notations are only present in the next section, and the non interested reader might directly go to \Cref{sec:experiments} for the application of the method above.

\begin{comment}
When using ULA for the SIS estimator, we can write explicitly the expression of the difference 
{\small\begin{multline} 
\sqrt{2\stepsize} \log\left( l_{k-1}(z_{k}, z_{k-1}) / m_k(z_{k-1}, z_k)\right) =\\ 
 \|z_k - z_{k-1} - \stepsize\nabla\log\unnormdistr_k(z_{k-1}) \|^2 - \|z_{k-1} - z_{k} - \stepsize\nabla\log\unnormdistr_k(z_{k}) \|^2 
\end{multline}}
\end{comment}


==> smc_old.tex <==


For some data $x\in\rset^N$, and parameter $\theta \in \mathsf{\Theta}$, consider the likelihood function
\begin{equation}
    p_\theta(x) = \int p_\theta(x, z)\rmd z\eqsp,
\end{equation}
where $z\in\rset^d$ are some latent variables.
Assume now that we have access to some unbiased estimator of the normalizing constant $p_\theta(x)$ of the unnormalized density $p_\theta(x,z)$, denoted $\hat{p}_\theta(x,z)$, that is 
\begin{equation}
    \int_{} \hat{p}_\theta(x,z) q_\phi(z\mid x) \rmd z = p_\theta(x)\eqsp.
\end{equation}
$\phi$ are here the parameters of the proposal distribution $q_\phi(z\mid x)$ used to compute the estimator $\hat{p}_\theta(x,z)$. We assume in the sequel that we have access to such a distribution. This is the typical setting of amortized Variational Inference.
We can build, based on Jensen's inequality, an Evidence Lower Bound using this estimator, writing
\begin{equation}
    \elbo = \int_{} \log \hat{p}_\theta(x,z) q_\phi(z\mid x) \rmd z \leq \log p_\theta(x)\eqsp.
\end{equation}
Moreover, it can be shown \cite{burda:grosse:2015, maddison2017filtering} that this bound becomes tighter as the variance of the estimator decreases. 



We specify in what follows two particular cases of interest for the computation of the weights.

% \subsection{Choosing reversible kernels, or Annealed Importance Sampling}

% Suppose here that the kernels $\{M_{k}\}_{k=1}^K, \{L_{k}\}_{k=0}^{K-1} $ satisfy, for $1\leq k\leq K$ $\unnormdistr_k(\rmd x)M_k(x,\rmd y)= \unnormdistr_k(\rmd y)L_{k-1}(y,\rmd x)$. Then, the expression of the weights boils down to
% \begin{equation}
%     \label{eq:weights_ais}
%     w_k(z_{k-1}, z_k) = w_k(z_{k-1}) =  \frac{\rmd\unnormdistr_t}{\rmd\unnormdistr_{t-1}}(z_{k-1})\eqsp.
% \end{equation}

\subsection{Bypassing the Accept-Reject with a stochastic flow}
We now take interest of non-reversible Markov kernels, that do not verify typically an invariance condition. This could be the case if we consider for example Unadjusted Langevin Algorithm (ULA) transformations, while Metropolis-Adjusted Langevin Algorithm would be its reversible counterpart.
Assume that the intermediate distribution have densities, also denoted $\{\unnormdistr_j\}_{j=0}^{K}$.
We can compute an estimator of the normalizing constant on two different ways
\subsubsection{Conditioning on the innovation noise}
\label{subsec:conditioned_stochastic_flows}
\achille{maybe these notations can be seen only after next section if we don't use this particular subsection without kernel densities}
Define a family of stochastic flows $\{\propmap{u,k}\,,\, u\in\msu\}_{k=1}^K$, assumed to be $\rmc^1$-diffeomorphisms, with $\msu = \rset^{D_u}$. The flows are said here, as they can be indexed by some innovation noise, with a density $\densinnovation$.
Define the deterministic conditional kernel and the associated Markov kernel $M_k$
\begin{align}
  \label{eq:indexed_kernel}
    &Q_{u,k}\bigl(z, \msa\bigr) = \updelta_{\propmap{u,k}(z)}(\msa) \eqsp, \\
    &M_k\bigl(z, \msa\bigr) = \int_\msu \updelta_{\propmap{u,k}(z)}(\msa) \densinnovation(u) \rmd u\eqsp.
  \end{align}
%A variable $U$ referred to as the \emph{innovation noise}, with density $h$
Define as well the reverse
\begin{align}
  \label{eq:indexed_kernel}
    &R_{u,k-1}\bigl(z, \msa\bigr) = \updelta_{\propmap{u,k}^{-1}(z)}(\msa) \eqsp, \\
    &L_{k-1}\bigl(z, \msa\bigr) = \int_\msu \updelta_{\propmap{u,k}^{-1}(z)}(\msa) \densinnovation(u) \rmd u\eqsp.
  \end{align}
Consider, for $\chunk{u}{1}{K}$, the kernels
$\{Q_{u,k}\}_{k=1}^K, \{R_{u,k}\}_{k=0}^{K-1}$, and the estimator based on these kernels.

We can write, for $1\leq k\leq K$, for non negative measurable functions $f,g$,
\begin{align}
\int \unnormdistr_k(\rmd z_k) R_{u_k,k-1}(z_k, \rmd z_{k-1})f(z_{k-1}) g(z_k) &=\int\unnormdistr_k( z_k) f(\propmap{u,k}^{-1}(z_{k}))g(z_k)\rmd z_k \\
&= \int\unnormdistr_k( \propmap{u,k}(z_{k-1}))f(z_{k-1})g(\propmap{u,k}(z_{k-1}))\Jac_{\propmap{u,k}}(z_{k-1})\eqsp.
\end{align}
Hence, we can write
$w_{u, k}(z_{k-1}, z_k) =w_{u, k}(z_{k-1})= \frac{\unnormdistr_k( \propmap{u,k}(z_{k-1}))}{\unnormdistr_{k-1}(z_{k-1})}\Jac_{ \propmap{u,k}}(z_{k-1})$.
We have
\begin{equation}
    \extendedfor(\rmd \chunk{z}{0}{K}) = \int_\msu \unnormdistr_0(\rmd z_0)\prod_{k=1}^K Q_{u,k}(z_{k-1},\rmd z_k)\densinnovation(\chunk{u}{1}{K}) \rmd \chunk{u}{1}{K}\eqsp,
\end{equation}
hence  if $\{\chunk{u^{(i)}}{1}{K}\}_{i=1}^{n}$ are sampled from $\densinnovation$ and $\{\chunk{z^{(i)}}{0}{K}\}_{i=1}^n$ are the $n$ independent trajectories from $\extendedfor$ associated, then
\begin{equation}
    \hat{\normconst} = \frac{1}{n} \sum_{i=1}^n \left[  \prod_{k=1}^{K}  w_{u_k^{(i)},k}(z_{k-1}^{(i)})\right]\eqsp.
\end{equation}
The weights in this estimators are associated to the innovation noise, which might not be a desirable property. However, with and additional assumption, we can simplify the expression of the estimator.
\subsubsection{Using the kernel densities}
Suppose now that the kernels $\{M_{k}\}_{k=1}^K, \{L_{k}\}_{k=0}^{K-1} $ admit tractable densities \wrt~ the Lebesgue measure, written $\{m_{k}\}_{k=1}^K, \{l_{k}\}_{k=0}^{K-1} $, for all $(x,y)\in\rset^{2d}$. This is the case typically for ULA (see \Cref{sec:supplementary} for derivation of the density and examples).

Then, we can easily write the expression of the weights and
\begin{equation}
    \label{eq:weights_with_density}
    w_k(z_{k-1}, z_k) = \frac{\unnormdistr_k(z_k)l_{k-1}(z_k, z_{k-1})}{\unnormdistr_{k-1}(z_{k-1})m_k(z_{k-1}, z_k)}\eqsp.
\end{equation}
In that case, the products of the weights simplifies, and we recognize in that case
\begin{equation}
    \label{eq:prod_weights_with_density}
    \prod_{k=1}^K w_k(z_{k-1}, z_k) = \frac{\unnormdistr_K(z_k)\prod_{k=1}^Kl_{k-1}(z_k, z_{k-1})}{\unnormdistr_{0}(z_{0})\prod_{k=1}^K m_k(z_{k-1}, z_k)}\eqsp.
\end{equation}
This is the general expression of the Hierarchical Variational Inference (HVI), in which $\prod_{k=1}^Kl_{k-1}(z_k, z_{k-1})$ are the ``reverse kernels'' that we usually want to find and optimize.

We would like to rely on this estimator to perform Variational Inference to learn parameters $\phi$ of the initial distribution $m$ and of parameters $\theta$ of the target distribution.

We now rely on the extension of \cite{thin:2020} to be able to differentiate the different estimators seen above.


\subsection{Hierarchical VAEs and CIF}
We do not consider anymore reversible kernels. Then, we separate our analysis here in two subsections.
\subsubsection{Conditioning on the innovation noise}
Recall that in this case, we can write explicitly the product of the weights as as a ratio between a deterministic pushforward and the target distribution.
\[\prod_{k=1}^K w_{u,k}(z_{k-1}, z_{k})  = \frac{p_\theta(x, z_K)}{q_\phi(z_0\mid x)}\Jac_{\Circ{t=1}{K}\propmap{t, u_t}}(z_{0})\eqsp.\] 
Then, we can write in this case
\begin{equation}
\elbosmc(\theta, \phi;x) =  \int q_\phi(z_0\mid x)  \densinnovation(\chunk{u}{1}{K}) \log\left(\left.p_\theta(x, \Circ{t=1}{K}\propmap{t, u_t}(z_{0}))\Jac_{\Circ{t=1}{K}\propmap{t, u_t}}(z_{0})\middle/q_\phi(z_0\mid x)\right.\right)\rmd z_0 \rmd \chunk{u}{1}{K}\eqsp.
\end{equation}

In particular, we can easily express the gradients \wrt $\phi, \theta$ with the reparameterization trick $V_{\phi,x}$, 
\begin{align}
    &\widehat{\nabla_\theta\elbosmc} = \nabla_\theta p_\theta(x, z_K)\,\text{ where }z_0 \sim q_\phi(z_0\mid x)\,,\,\chunk{u}{1}{K}\sim \densinnovation \,,\, z_K=\Circ{t=1}{K}\propmap{t, u_t}(z_{0})\\
    &\widehat{\nabla_\phi\elbosmc} = \nabla_\phi \left[\log p_\theta(x, \Circ{t=1}{K}\propmap{t, u_t}(V_{\phi,x}(\epsilon)) - \log q_\phi(V_{\phi,x}(\epsilon)\mid x) + \log \Jac_{\Circ{t=1}{K}\propmap{t, u_t}}(V_{\phi,x}(\epsilon))\right]\,,\, \epsilon\sim \densgauss\,,\, \chunk{u}{1}{K}\sim \densinnovation\eqsp.
\end{align}
We recognize a noisy estimator of the VAE with normalizing flows, due to the fact that we are using here stochastic flows.


==> smc_vae.tex <==


\subsection{Langevin VAE}

We define here the Langevin VAE, which implements annealed Langevin dynamics in the setting described above. 
Define thus $\{m_{k}\}_{k=1}^K, \{l_{k}\}_{k=0}^{K-1} $
the families of Markov transitions, densities associated to the proposal mappings $\{\propmap{t, u}\}_{1\leq t\leq K, u\in\msu}$ and the innovation noise with density $\densinnovation$.
Suppose that we also have access to the densities . Then,
\begin{multline}
\elbosmc(\theta, \phi;x) =  \int q_\phi(z_0\mid x)  \densinnovation(\chunk{u}{1}{K}) \\\log\left(\frac{p_\theta(x, z_K)\prod_{k=1}^K l_{k-1}(z_k, z_{k-1})}{q_\phi(z_0\mid x)\prod_{k=1}^K m_k(z_{k-1}, z_k)}\right)\rmd z_0 \rmd \chunk{u}{1}{K}\eqsp,
\end{multline}
where we used the short-hand notation for $k\leq K$, $z_k= \Circ{t=1}{k}\propmap{t, u_t}(z_{0})$. An estimator of this ELBO is  obtained easily and given by sampling $z_0\sim q_\phi(\cdot\mid x), \, \chunk{u}{1}{K}\sim \varphi$, and setting recursively $z_k = \propmap{k, u_k}(z_{k-1})$.
Note that when we use Langevin dynamics, our transitions are inherently amortized as they convey the gradient of $\unnormdistr_{k, x}$.
The gradient of this ELBO can also be easily estimated, using in particular the reparameterization trick, see Supplementary for more details.


\begin{comment}
\paragraph{Score matching}

In practice, we might not want to compute the gradient of $\unnormdistr_k(z\mid x) = q_\phi(z\mid x)^{1-\beta_k} p_\theta(x, z)^{\beta_k}$ in order to have a computationally cheaper algorithm.\textcolor{red}{why would we not compute it in our context?}

Instead, inspired by score matching techniques, which have proven state of the art results on sampling experiments, we introduce an additional network, denoted $s_\psi(x, z, \beta)$.

The transformation $\propmap{k,u}$ now becomes
\begin{equation}
    \propmap{k,u}(z) = z + \diag{\stepsize} * s_\psi(x, z, \beta_k) + \sqrt{2\diag{\stepsize}} u\eqsp.
\end{equation}
Note that we write here $\diag{\stepsize}$ as we might want different values of $\stepsize$ on the different coordinates. 
As in score matching, we consider another objective to learn the parameters $\psi$, that is
\begin{equation}
    \elbo_{\scorematching}(\psi; x) = \PE_{Q} \left[\sum_{k=1}^K \|s_\psi(x, z_k, \beta_k) - \nabla_z \log \unnormdistr_k(z_k \mid x)\|^2\right]
\end{equation}
\end{comment}

